The Roles of Symbols in Neural-based AI: They are Not What You Think!

We propose that symbols are first and foremost external communication tools used between intelligent agents that allow knowledge to be transferred in a more efficient and effective manner than having to experience the world directly. But, they are also used internally within an agent through a form of self-communication to help formulate, describe and justify subsymbolic patterns of neural activity that truly implement thinking. Symbols, and our languages that make use of them, not only allow us to explain our thinking to others and ourselves, but also provide beneficial constraints (inductive bias) on learning about the world. In this paper we present relevant insights from neuroscience and cognitive science, about how the human brain represents symbols and the concepts they refer to, and how today's artificial neural networks can do the same. We then present a novel neuro-symbolic hypothesis and a plausible architecture for intelligent agents that combines subsymbolic representations for symbols and concepts for learning and reasoning. Our hypothesis and associated architecture imply that symbols will remain critical to the future of intelligent systems NOT because they are the fundamental building blocks of thought, but because they are characterizations of subsymbolic processes that constitute thought.

==> chapter-dummy/chap.tex <==
\chapter{Chapter  Title : Dummy}
\label{chapter-dummy:chap}
\chapterauthor{Firstname1 Lastname1}{Affiliation1 Affiliation1 Affiliation1 Affiliation1 Affiliation1 Affiliation1 Affiliation1}
\chapterauthor{Firstname2 Lastname2}{Affiliation2}
\chapterauthor{Firstname3 Lastname3}{Affiliation2}

\allchapterauthors{Firstname1 Lastname1, Firstname2 Lastname2, Firstname3 Lastname3}

Dic nam esta pulchra ut luna electa, ut sol replet laetitia terras,
caelos. Maria virgo illa dulcis, praedicata de propheta porta
orientalis. Nigra sum, sed for-mosa, filiae. Ideo dilexit me rex et
introduxit me in cubiculum suum et dixit mihi. Surge, amica mea, et
veni. Iam hiems transiit, imber abiit et recessit, flores apparuerunt in
terra nostra. Audi caelum, verba mea, plena desiderio et perfusa gaudio. \cite{DBLP:conf/iceis/BlomqvistS05}


\section{Short Head One}

Isi aedificaverit domum \cite{JainHYVS10,gruber95}, in vanum \cite{gangemi2005} laboraverunt qui aedificant eam.
Nisi custo-dierit civitatem, frustra vigilat qui custodit eam. Vanum
est vobis ante lucem surgere: surgite postquam sederitis, qui
manducatis panem doloris. Cum dederit dilectis suis somnum: ecce
haereditas filii: merces, fructus ventris. Sicut sagit-tae in many
potentis: ita filii excussorum. Beatus vir qui implevit desiderium
suum ex pisis: non confundetus cum loquetur inimicis suis in porta.
Ideo dilexit me rex et introduxit me in cubiculum suum et dixit mihi.
Surge, amica mea, et veni. \ref{chapter1:chap}

\subsection{Short Head Two}

Dic nam esta pulchra ut luna electa, ut sol replet laetitia terras,
caelos. Maria virgo illa dulcis, praedicata de propheta porta
orientalis. Nigra sum, sed for-mosa, filiae. Ideo dilexit me rex et
introduxit me in cubiculum suum et dixit mihi. Surge, amica mea, et
veni. Iam hiems transiit, imber abiit et recessit, flores apparuerunt in
terra nostra. Audi caelum, verba mea, plena desiderio et perfusa gaudio.



\begin{table}[t]

\caption{Table caption could be very long.}

\begin{tabular}{lp{5cm}}
\hline
First &       \\ Line  & Second \\ \hline First  &
Nationi, et iudicia sua non manifestavit eis. Et exultavit
spiritus meus
                    in salutari meo.\\

Second & Et misericordia eius a progenie\\
\hline
\end{tabular}
\end{table}


\begin{table}[t]

\caption{Table caption could be very long.
Dic, quaeso, mihi: quae est ista, quae consurgens ut aurora rutilat
ut beneficam}

\begin{tabular*}{0.9\textwidth}{ll}
\hline
First &       \\ Line  & Second \\ \hline First  &
Nationi, et iudicia sua non manifestavit eis. Et exultavit
spiritus meus
                    in salutari meo.\\

Second & Et misericordia eius a progenie\\
\hline
\end{tabular*}
\end{table}




\begin{figure}[t]
\vspace*{40mm}

\caption{%
Nisi custodierit civitatem, frustra vigilat qui custodit eam. Vanum
est vobis ante lucem surgere: surgite postquam sederitis, qui
manducatis panem doloris.}
\end{figure}

\begin{figure}[t]
\vspace*{40mm}
\caption{Nisi custodierit civitatem}
\end{figure}

\bibliographystyle{tfnlm}
\bibliography{chapter-dummy/reference}
